Towards Good Practices in Evaluating Transfer Adversarial Attacks

Transfer adversarial attacks raise critical security concerns in real-world, black-box scenarios. However, the actual progress of this field is difficult to assess due to two common limitations in existing evaluations. First, different methods are often not systematically and fairly evaluated in a one-to-one comparison. Second, only transferability is evaluated but another key attack property, stealthiness, is largely overlooked. In this work, we design good practices to address these limitations, and we present the first comprehensive evaluation of transfer attacks, covering 23 representative attacks against 9 defenses on ImageNet. In particular, we propose to categorize existing attacks into five categories, which enables our systematic category-wise analyses. These analyses lead to new findings that even challenge existing knowledge and also help determine the optimal attack hyperparameters for our attack-wise comprehensive evaluation. We also pay particular attention to stealthiness, by adopting diverse imperceptibility metrics and looking into new, finer-grained characteristics. Overall, our new insights into transferability and stealthiness lead to actionable good practices for future evaluations.

==> tex/10imagesEachAttack.tex <==
% \clearpage
% \newpage

% \section{Visualizations of Adversarial Examples}
% \label{app:vis}


\begin{figure*}[t]
\newcommand{\sizeS}{.095}
\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{figures/visualize_examples/#2}}
\tiny
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{rccccccccccc}

Original&
\fig[\sizeS]{clean_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{clean_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{clean_ILSVRC2012_val_00047539_pt.png} \\

PGD&
\fig[\sizeS]{baseline_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{baseline_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{baseline_ILSVRC2012_val_00047539_pt.png} \\

MI&
\fig[\sizeS]{MI_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{MI_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{MI_ILSVRC2012_val_00047539_pt.png} \\

NI&
\fig[\sizeS]{NI_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{NI_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{NI_ILSVRC2012_val_00047539_pt.png} \\

PI&
\fig[\sizeS]{PI_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{PI_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{PI_ILSVRC2012_val_00047539_pt.png} \\


\end{tabular}
\caption{Adversarial examples generated by gradient stabilization attacks, along with original images and the baseline PGD attack.}
\label{fig:10adv-show-1}
% \vspace{-0.8cm}
\end{figure*}

\begin{figure*}[t]
\newcommand{\sizeS}{.095}
\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{figures/visualize_examples/#2}}
\tiny
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{rccccccccccc}

DI&
\fig[\sizeS]{DI_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{DI_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{DI_ILSVRC2012_val_00047539_pt.png} \\

TI&
\fig[\sizeS]{TI_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{TI_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{TI_ILSVRC2012_val_00047539_pt.png} \\

SI&
\fig[\sizeS]{SI_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{SI_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{SI_ILSVRC2012_val_00047539_pt.png} \\

VT&
\fig[\sizeS]{VT_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{VT_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{VT_ILSVRC2012_val_00047539_pt.png} \\

Admix&
\fig[\sizeS]{Admix_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{Admix_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{Admix_ILSVRC2012_val_00047539_pt.png} \\

\end{tabular}
\caption{Adversarial examples generated by input augmentation attacks.}
\label{fig:10adv-show-2}
\end{figure*}

\begin{figure*}[t]
\newcommand{\sizeS}{.095}
\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{figures/visualize_examples/#2}}
\tiny
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{rccccccccccc}

TAP&
\fig[\sizeS]{TAP_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{TAP_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{TAP_ILSVRC2012_val_00047539_pt.png} \\

AA&
\fig[\sizeS]{AA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{AA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{AA_ILSVRC2012_val_00047539_pt.png} \\

ILA&
\fig[\sizeS]{ILA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{ILA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{ILA_ILSVRC2012_val_00047539_pt.png} \\

FIA&
\fig[\sizeS]{FIA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{FIA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{FIA_ILSVRC2012_val_00047539_pt.png} \\

NAA&
\fig[\sizeS]{NAA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{NAA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{NAA_ILSVRC2012_val_00047539_pt.png} \\

\end{tabular}
\caption{Adversarial examples generated by feature disruption attacks.}
\label{fig:10adv-show-3}
\end{figure*}

\begin{figure*}[t]
\newcommand{\sizeS}{.095}
\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{figures/visualize_examples/#2}}
\tiny
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{rccccccccccc}

SGM&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{data_resnet50_SGM_ILSVRC2012_val_00047539_pt.png} \\

LinBP&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{data_resnet50_LinBP_ILSVRC2012_val_00047539_pt.png} \\

RFA&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{data_resnet50_RFA_ILSVRC2012_val_00047539_pt.png} \\

IAA&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{data_resnet50_IAA_ILSVRC2012_val_00047539_pt.png} \\

DSM&
\fig[\sizeS]{dark_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{dark_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{dark_ILSVRC2012_val_00047539_pt.png} \\

\end{tabular}
\caption{Adversarial examples generated by surrogate refinement attacks.}
\label{fig:10adv-show-4}
\end{figure*}


\begin{figure*}[t]
\newcommand{\sizeS}{.095}
\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{figures/visualize_examples/#2}}
\tiny
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{rccccccccccc}

GAP&
\fig[\sizeS]{GAP_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{GAP_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{GAP_ILSVRC2012_val_00047539_pt.png} \\

CDA&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{data_resnet152_CDA_ILSVRC2012_val_00047539_pt.png} \\

GAPF&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{data_resnet152_GAPF_ILSVRC2012_val_00047539_pt.png} \\

BIA&
\fig[\sizeS]{BIA_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{BIA_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{BIA_ILSVRC2012_val_00047539_pt.png} \\

TTP&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00025507_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00018792_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00023023_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00030598_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00036281_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00042464_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00043962_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00044685_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00045149_adv.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00047539_adv.png} \\
&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00025507_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00018792_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00023023_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00030598_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00036281_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00042464_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00043962_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00044685_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00045149_pt.png}&
\fig[\sizeS]{TTP_5000_ILSVRC2012_val_00047539_pt.png} \\

\end{tabular}
\caption{Adversarial examples generated by generative modeling attacks.}
\label{fig:10adv-show-5}
\end{figure*}



